Flash: An Asynchronous Payment System with Good-Case Linear Communication Complexity

While the original purpose of blockchains was to realize a payment system, it has been shown that, in fact, such systems do not require consensus and can be implemented deterministically in asynchronous networks. State-of-the-art payment systems employ Reliable Broadcast to disseminate payments and prevent double spending, which entails O(n^2) communication complexity per payment even if Byzantine behavior is scarce or non-existent. Here we present Flash, the first payment system to achieve $O(n)$ communication complexity per payment in the good case and $O(n^2)$ complexity in the worst-case, matching the lower bound. This is made possible by sidestepping Reliable Broadcast and instead using the blocklace -- a DAG-like partially-ordered generalization of the blockchain -- for the tasks of recording transaction dependencies, block dissemination, and equivocation exclusion, which in turn prevents doublespending. Flash has two variants: for high congestion when multiple blocks that contain multiple payments are issued concurrently; and for low congestion when payments are infrequent.

==> Code/blocklace-mobile.tex <==
\begin{figure}[pt]
\begin{algorithm}[H]
    \caption{\textbf{\msys: Blocklace Utilities.} Code for miner $p $}
    \label{alg:blocklace}
    \small
    \begin{changemargin}{0cm}{-2cm}
    \begin{algorithmic}[1] \scalefont{0.9}
        % \begin{multicols}{2}
        % \State \oded{I've decreased the font size for the algorithm to fit in.}
        \Statex \textbf{Local variables:}
        \StateX struct $\textit{block } b$: \Comment{The structure of a block $b$ in a blocklace, Def.\ \ref{definition:block}}
        % \StateXX $b.\textit{round}$ - the round of $v$ in the DAG
        \StateXX $b.\textit{creator}$ -- the miner that created $b$ 
         \StateXX $b.\textit{address}$ -- address of $b.\textit{creator}$
        \StateXX $b.\textit{payload}$ -- a set of transactions
  %      \StateXX $b.\textit{share}$ -- a share of the random coin, if needed 
        \StateXX $b.\textit{pointers}$ -- a possibly-empty set of hash pointers to other blocks
        \StateX \textit{blocklace} $\gets \{\}$  \Comment{The local blocklace of miner $p$}
	  
		
% 		\vspace{0.5em}
		\Procedure{$\textit{create\_block}$}{\textit{payload}}: %\oded{Add an if condition to make sure $d$ is the maximal round of the blocklace.}\udi{I don't think it is needed; in factn it can be called with infinity and still work.  The protocol uses it in a specific way, which is fine.}
		%\Comment Add to \emph{blocklace} a new block $b$ with \textit{payload} and pointers to the roots of \emph{blocklace}
		\State \textbf{new} $b$  \Comment{Allocate a new block structure}
		\State $b.\textit{creator} \gets p$
        \State $b.\textit{address} \gets \textbf{current\_address}()$ 
        \Comment{Returns current address of $p$}
		\StateX $b.\textit{payload} \gets \textit{payload}$ 
     
        \State $b.\textit{pointers} \gets hash(roots)$, \text{where} \textit{roots} 
  \text{are the roots of} \textit{blocklace}, \text{including the last $p$-block}\label{alg:roots} \Comment{Def. \ref{definition:closure}}
	   %   \State $\textit{blocklace} \gets \textit{blocklace}~ \cup \{ b\}$ 	
	   %   \State $\tau()$ \Comment{\Cref{section:tau}, \Cref{alg:tau-def}} \label{alg:CMA:addedOutgoingBlock}
	      \State \Return $b$
		\EndProcedure
		
		
        % \vspace{0.5em}
		\Procedure{\textit{hash}}{$b$}:
	    \Return collision-free cryptographic hash pointer to block $b$ %\Comment{Returns a set if applied to a set}
        \EndProcedure
        
		
        % \vspace{0.5em}
        \Procedure{$b\succeq b'$}{}: \Comment{Def.\ \ref{definition:observe}} 
        \State \Return $\exists b_1,b_2,\ldots,b_k \in \textit{blocklace}$, $k\ge 1$,  s.t.\
        $b_1 = b $, $b_k = b'$ and $\forall i \in [k-1] \colon \textit{hash}(b_{i+1}) \in b_i.\textit{pointers}$
        \EndProcedure
        
        
        
        
        % \vspace{0.5em}
        \Procedure{\textit{closure}}{$B$}: \label{alg:SMR:closure} 
         \Return $\{b' \in \textit{blocklace} : b \in B \wedge b\succeq b'\}$ \Comment{Def.  \ref{definition:closure}. Also referred to as $[B]$. If $B=\{b\}$ is a singleton we use $[b]$ instead of $[\{b\}]$.}
        %\oded{Don't understand what ``called via [b]'' means}
        \EndProcedure
       
      
% 		\vspace{0.5em}  
	    \Procedure{\textit{equivocation}}{$b_1,b_2$}: \label{alg:SMR:da}
            \Return 
            $b_1.\textit{creator} = b_2.\textit{creator} \wedge
            b_1 \not\succeq b_2 \wedge
            b_2 \not\succeq b_1
           $ \Comment{Def.\ \ref{definition:equivocation}, Fig. \ref{figure:approve-sr}.A} 
           %\oded{Why not use the closure function?}
           % \udi{ [b] = closure(b)}
        \EndProcedure
		
		
% 		\vspace{0.5em}  
	    \Procedure{\textit{equivocator}}{$q,b$}: \label{alg:SMR:dactor}
            \State \Return 
            $\exists b_1,b_2 \in [b] \wedge
            b_1.\textit{creator} = b_2.\textit{creator} = q \wedge
          \textit{equivocation}(b_1,b_2)
           $ \Comment{Def.\ \ref{definition:equivocation}, Fig. \ref{figure:approve-sr}.A}
        \EndProcedure
        
        
        % 	 \vspace{0.5em}	
		\Procedure{\textit{approves}}{$b,b_1$}: \label{alg:SMR:approves}
            \Return $b_1 \in [b]  \wedge \forall b_2 \in [b] : \lnot$\textit{equivocation}$(b_1,b_2)$  \Comment{Def.\ \ref{definition:approval}, Fig. \ref{figure:approve-sr}.A}
        \EndProcedure
          
      
% 		 \vspace{0.5em}	
		\Procedure{\textit{ratifies}}{$b_1,b_2$}: \Comment{Def.\ \ref{definition:ratified-block}, Fig. \ref{figure:approve-sr}.B} \label{alg:ratifies} 
         \State \Return
            $   \textit{approves}(b1,b_1) \wedge
            \{b.\textit{creator} : b \in [b_1]   \wedge
               \textit{approves}(b1,b) \wedge \textit{approves}(b,b_2) \}$
            is a supermajority 
            \EndProcedure
       
            
      
% 		 \vspace{0.5em}	
		\Procedure{\textit{super\_ratifies}}{$B_1,b_2$}: \label{alg:super-ratifies} 
		\Comment{Def.\ \ref{definition:ratified-block}, Fig. \ref{figure:approve-sr}.C}
         \State \Return
            $
            \{b.\textit{creator} : b \in [B_1]   \wedge
              \textit{ratifies}(b,b_2) \}$
            is a supermajority 
            \EndProcedure
       
       
       
        
	
        % \vspace{0.5em}
        \Procedure{\textit{height}}{$b$}:
        \Return max~ $\{k : \exists b' \in$ \textit{blocklace} with a path from $b$ to $b'$ of length $k$\}. \Comment{Def.~\ref{definition:height}}
         \EndProcedure
        
        
         %\vspace{0.5em}
        \Procedure{\textit{blocklace\_prefix}}{$d$}:
        \Return  $\{b \in \textit{blocklace} : \textit{height}(b) \le d\}$  \Comment{Def.\ \ref{definition:height}}
        \EndProcedure
        
        %\vspace{0.5em}
        
        % \vspace{0.5em}
        \Procedure{\textit{address}}{$q,B$}:  \Comment{See Def. XXX}
        \State $ b \gets \text{ tallest $q$-block in $B$}$ 
        \State \Return    $b.\textit{address}$ else $\textit{initial\_address}(q)$ \Comment{For bootstrap, we assume that at least one miner initially knows the current addresses of the others.}
          
        \EndProcedure
        
        % \vspace{0.5em}
        \Procedure{\textit{cordial\_block}}{$b,B$}:  \Comment{See Def. \ref{definition:cordial}}
        \State $ b' \gets \text{ tallest block in $B$ for which } b.\textit{creator} = b'.\textit{creator}$
        \State \Return   $\{b''.\textit{creator} :  b \succ b'' \succ b'\}$ is a            supermajority $\vee$  
            $b.\textit{address} \ne b'.\textit{address}$ 
            \Comment{Address change trumps cordiality}
        \EndProcedure
        
        
        
        
        
        %\Procedure{\textit{round}}{\textit{blocks}} 
        %\Return $\max~ \{\textit{round}(b) : b \in \textit{blocks}\}$ \Comment{Depth of set of blocks}
        %\EndProcedure
        
	    
        
    
        %\vspace{0.5em}
        %\Procedure{\textit{leaders}}{\textit{blocks}} 
        %\Return $\{b \in \textit{blocks} : b.\textit{creator} = \textit{leader}(\textit{round}(b))\}$
        %\EndProcedure
        
        
          
        \alglinenoNew{counter}
        \alglinenoPush{counter}
    % \end{multicols}
 
    \end{algorithmic}
      \end{changemargin}
\end{algorithm}
\vspace{-2.5em}
\end{figure}

==> Code/dissemination-UDP.tex <==
\begin{figure}[tp]
\begin{algorithm}[H]
	\caption{\textbf{Grassroots Cordial Dissemination for Mobile Agents Over UDP}\\ Code for agent $p$, including Algorithm \ref{alg:blocklace}}	\label{alg:GCD-UDP}
	%\small
	%\begin{changemargin}{0cm}{-1.5cm}
	\begin{algorithmic}[1] \scalefont{0.93}
	\alglinenoPop{counter} 
		

	\Statex \textbf{Local variables:}
    \StateX \textit{timer} \Comment{with \textbf{reset} and \textbf{timeout} operations}
    \StateX $\textit{my\_ip} \gets \bot$ \Comment{My IP address and open UDP port, updated externally}
\vspace{0.5em}

     	\Upon{change to \textit{my\_ip}}     \label{alg:disseminate-new-IP}
	            \Comment{Update friends of my new address}
        \State  $b\gets \{\textit{create\_block}((\textit{`ip\_address'},\textit{my\_ip}))\}$
	    \EndUpon

\vspace{0.5em}
	\Upon{decision to send $b \in \textit{blocklace}$ to address \textit{IP}}   \label{alg:BDA-b-to-q}   \Comment{Decision made externally} 
       \State  \textbf{send}  $b$ to \textit{IP}   \Comment{2. \textbf{Send-$b$-to-$q$}}
	 \EndUpon

  
\vspace{0.5em}

	\Upon{$\textbf{receive } b$}   \label{alg:BDA-receive}   \Comment{3. \textbf{Receive-$b$}}
	  \State  $\textit{blocklace}\gets \textit{blocklace} \cup \{b\}$  \label{alg:BDA-receive}
	 \EndUpon

  
	   	 \vspace{0.5em}	
     	\Upon{$\textbf{timeout}(\textit{timer})$}     \label{alg:disseminate-timeout}
	            \Comment{4. \textbf{Cordially-Send-$b$-to-$q$}}
        \For{all $b\in \textit{blocklace}, q \in P :  \textit{friend}(q) \wedge \textit{follows}(q, b.\textit{creator}) \wedge \lnot\textit{agentObserves}(q,b)$}
	    \State \textbf{send}  $b$ to  $ip(q)$  \label{alg:send-package}
	    \EndFor
     	\State $\textbf{reset}(\textit{timer})$ \label{alg:reset-upon-send-package}
	    \EndUpon

   
\vspace{0.5em}
        \Procedure{$\textit{ip}(q)$}{} \Comment{Most-recently known IP address of $q$} 
        \State Let $b$ be the most recent $q$-block in \textit{blocklace} s.t. $b.\textit{payload}= (\textit{`ip\_address'},\textit{IP})$ 
        \State \Return $\textit{IP}$ 
        \EndProcedure
        

		\alglinenoPush{counter}
	\end{algorithmic}
	
          
	
	%\end{changemargin}
% 	\vspace{-5em}
\end{algorithm}
\vspace{-2em}
\end{figure}



==> Code/dissemination-laconic.tex <==
\begin{figure}[tp]
\begin{algorithm}[H]
	\caption{\textbf{Laconic Dissemination}\\ Code for miner $p$
 %, including Algorithms \ref{alg:blocklace}, \ref{alg:utilities}, \ref{alg:tau}
 }
 \label{alg:lm}
%	\small
	\begin{changemargin}{0cm}{-1.5cm}
	\begin{algorithmic}[1] \scalefont{0.93}
	\alglinenoPop{counter} 
		

	\Statex \textbf{Local variables:}
	 \StateX array $\textit{timer}(n)$ \Comment{A timer for each $q \in \Pi$ with \textbf{reset} and \textbf{timeout}, initially reset} 
	 \StateX \textit{payload} $\gets \bot$  \Comment{Updated externally}
  %     \StateX \textit{approvals} $\gets \emptyset$  \Comment{Pending Approvals}
       \StateX \textit{buffer} $\gets \emptyset$  \Comment{Pending incoming blocks}
       \StateX \textit{blocklace} $\gets \emptyset$  \Comment{Local blocklace}
      
 \vspace{0.5em}

	\Upon{$\textit{payload} \ne \emptyset$}   \label{alg:cordially-ready}   \Comment{1. \textbf{Send}}
    \State wait according to exponential backoff
	\State $b \gets \textit{create\_block}(\textit{payload})$  \label{alg:create-next-block}
			\For{$q \in \Pi$} 
		        \State  \textbf{send}  $b$ to $q$  \label{alg:send-block-to-others}
		       	\State $\textbf{reset}(\textit{timer}(q))$
		   \EndFor
	   \State $\textit{payload}\gets \bot$
	 \EndUpon
	 
	 \vspace{0.5em}
    \Upon{$\textit{rejected}(x,\textit{blocklace}) \wedge \textit{payload} = \bot$} \Comment{\textbf{Retransmit rejected payload}}
    \State $\textit{payload}\gets x$ 
    \EndUpon

	 \vspace{0.5em}
    \Upon{$\textit{accepted}(x,\textit{blocklace}) \wedge x \ne \emptyset$} \Comment{\textbf{4. Output}}
    \State $\textbf{output}(x)$ 
    \EndUpon

 \vspace{0.5em}	
 
	\Upon{$\textbf{receive } b$, $b \notin \textit{buffer} \cup blocklace$}   \label{alg:BDA-receive} \Comment{\textbf{Buffer block}}   
   
	    \State $\textit{buffer}\gets \textit{buffer} \cup \{b\}$  \label{alg:BDA-receive}

	 \EndUpon

	 
	\vspace{0.5em}	

	\While{$b \in \textit{buffer} \wedge \textit{closed}(\textit{blocklace} \cup \{b\})$}\label{alg:buffer}  \Comment{2. \textbf{Receive}}
  \If{$\textit{conflicting}(b,\textit{blocklace})$}
    \State $\textit{send\_approval}()$
      \EndIf
    \State $\textit{blocklace} \gets \textit{blocklace} \cup \{b\}$,
             $\textit{buffer} \gets \textit{buffer} \setminus \{b\}$,
             \label{alg:blocklace-follow-qa}  
    \If{$\textit{conflicting}(b,\textit{blocklace})$}
    \State $\textit{send\_approval}()$
      \EndIf
 \EndWhile

 \vspace{0.5em}	

	
	 
	 \vspace{0.5em}
 

	     \Upon{\textbf{timeout}$(\textit{timer}(q))$} \label{alg:disseminate-timeout}
	    \label{alg:timeout} 	 \Comment{3. \textbf{Cordial dissemination}}
	       \State \textit{Let} $b_q \in \textit{blocklace}$ be the last $q$-block known to $p$
            \For{$b \in  \textit{blocklace} \setminus [b_q] $} 
                \textbf{send}  $b$ to  $q$  \label{alg:send-package}
            \EndFor
	    \State $\textbf{reset}(\textit{timer}(q))$ \label{alg:reset-upon-send-package}
        \EndUpon 
	  

        
         \vspace{0.5em}
        \Procedure{\textit{send\_approval}}{} %\Comment{Def. Rejected} 
        \State $b \gets \textit{create\_block}(\emptyset)$  \label{alg:create-next-block}
			\For{$q \in \Pi$} 
		        \State  \textbf{send}  $b$ to $q$  \label{alg:send-block-to-others}
		       	\State $\textbf{reset}(\textit{timer}(q))$
          \EndFor
        \EndProcedure
        


        
         \vspace{0.5em}
        \Procedure{\textit{accepted}}{$b$,\textit{blocklace}}: \Comment{Def. Accepted} 
        %\Return $\exists b'\in \textit{blocklace} \wedge \textit{final}(b') \wedge b.\textit{time} < b'.\textit{time} \wedge b'\not\succ b$
        \EndProcedure
        
         \vspace{0.5em}
        \Procedure{\textit{rejected}}{$b$,\textit{blocklace}}: \Comment{Def. Rejected} 
        %\Return $\exists b'\in \textit{blocklace} \wedge \textit{final}(b') \wedge b.\textit{time} < b'.\textit{time} \wedge b'\not\succ b$
        \EndProcedure
        
         \vspace{0.5em}
        \Procedure{\textit{conflicting}}{$b$,\textit{blocklace}}: \Comment{Def. Conflicting} 
        %\Return $\exists b'\in \textit{blocklace} \wedge \textit{final}(b') \wedge b.\textit{time} < b'.\textit{time} \wedge b'\not\succ b$
        \EndProcedure
        







        
		\alglinenoPush{counter}
	\end{algorithmic}
	
          
	
	\end{changemargin}
% 	\vspace{-5em}
\end{algorithm}
\vspace{-2em}
\end{figure}



==> Code/dissemination.tex <==
\begin{figure}[t]
\begin{algorithm}[H]
	\caption{\textbf{\sys:  Dissemination}\\ Code for miner $p$, including Algorithms \ref{alg:blocklace},  \ref{alg:tau} \&  \ref{alg:utilities}}	\label{alg:dissemination}
	\small
	\begin{changemargin}{0cm}{-1.5cm}
	\begin{algorithmic}[1] \scalefont{0.93}
	\alglinenoPop{counter} 
		

	\Statex \textbf{Local variables:}
	 \StateX array $\textit{timer}(n)$ \Comment{A $\Delta$-timer for each $q \in \Pi$, with $\textbf{reset}(\textit{timer}(q))$ and \textbf{timeout}(\textit{timer}(q))} 
	 

	 \For{$q \in \Pi \setminus \{p\}$} \Comment{Background cordial dissemination by $p$ to all other miners}
		        \State  $||$ \textit{disseminate\_to}$(q)$  \label{alg:call-disseminate} 
	\EndFor
	\vspace{0.5em}	
	\Upon{cordially\_ready}   \label{alg:cordially-ready}
	    \State $b \gets \textit{create\_block}()$  \label{alg:create-next-block} \Comment{$b$ is cordial}
			\For{$q \in \Pi$} 
		        \State  \textbf{send}  $\{b\}^p$ to $q$  \label{alg:send-block-to-others}
		       	\State $\textbf{reset}(\textit{timer}(q))$
		   \EndFor
	   
	 \EndUpon
	 
	 
	\vspace{0.5em}	 
	\Upon{\textbf{receiving} $B_q$}
	    \label{alg:receive} 
	\If{$\textit{cordial}(\textit{blocklace} \cup B)$} \label{alg:cordial-blocklace}
	\State $\textit{blocklace} \gets \textit{blocklace} \cup B$ \label{alg:blocklace-adds-B}
	\State $\tau()$ \label{alg:call-tau} 
	\State $\textbf{reset}(\textit{timer}(q))$  \label{alg:reset-timer-q-upon-receipt} 
	\EndIf
	\EndUpon
	
    

		
        %\vspace{0.5em}
        %\Procedure{$\textit{can\_proceed}()$}{}
        % \Return  $ r \in \textit{cordial\_round}() 
        %\wedge (timer \ge \Delta \vee \textit{leader}(r))$
        %\Comment{Instance for eventual synchrony}
        
	
	
	   	 \vspace{0.5em}	
		\Procedure{\textit{disseminate\_to}}{$q$} \label{alg:disseminnate}  \Comment{Cordial dissemination}
     	\Upon{\textbf{timeout}$(\textit{timer}(q))$} \label{alg:disseminate-timeout}
	    \label{alg:timeout} 
	    \If{\textit{blocklace} has a $p$-block not observed by any $q$-block} \label{alg:check-for-q-block}
	    \State $b_q \gets$ highest $q$-block in \textit{blocklace}
	    \State $b_p \gets$ lowest $p$-block in \textit{blocklace} that observes $b_q$
	    \State \textbf{send}  $([b_p] \setminus [b_q])^p$ to  $q$  \label{alg:send-package}
	    \State $\textbf{reset}(\textit{timer}(q))$ \label{alg:reset-upon-send-package}
	    \EndIf
	    \EndUpon
	  	\EndProcedure
	  	
        	
         \vspace{0.5em}
        \Procedure{\textit{cordial}}{$B$}  \Comment{See Def. \ref{definition:cordial}}
        \label{alg:cordial-B}
        \State \Return  $B = [B] \wedge (\forall b \in B: \textit{cordial(b,B)})$
        \EndProcedure
        
       
        	
         \vspace{0.5em}
        \Procedure{\textit{cordially\_ready}}{}  
        \label{alg:ready}
        \State \Return $b \gets$ highest $p$-block $\in \textit{blocklace} \implies$
        \State $\{b'.\textit{creator}: b'\in \textit{blocklace} \wedge b' \succ b \}$ is a supermajority
        \EndProcedure
        
        
        
		\alglinenoPush{counter}
	\end{algorithmic}
	
          
	
	\end{changemargin}
% 	\vspace{-5em}
\end{algorithm}
\vspace{-2em}
\end{figure}



==> Code/protocols.tex <==
\begin{figure}[t]

\begin{algorithm}[H]
	\caption{\textbf{\sys:  Probabilistic Synchrony.} \\
	Code for miner $p$}
	\label{alg:utilities}
	%\small
	 \begin{changemargin}{0cm}{-2cm}
      \begin{algorithmic}[1] 
      \alglinenoPop{counter} 
                
        \State $w \gets 3$ \label{alg:w-3}     
        
       \Procedure{\textit{leader}}{$d$}:  \label{alg:leader} 
        \Return $q \in \Pi$ selected deterministically if $d \text{ mod } w = 0$ else $\bot$. 
        \EndProcedure
        
        
        % \vspace{0.5em}
        \Procedure{\textit{final\_leader}}{$b$}: \label{alg:finalLeader} \Comment{$b$ is super-ratified within $d+w-1$ or ratified by its $d+w$ successor and super-ratified within $d+w$, Def. \ref{definition:final-leaders}}
        \State \Return $d = \textit{height}(b) \wedge 
        \textit{leader}(d) = b.\textit{creator}~ \wedge $
        \State $\textit{blocklace\_prefix}(d+w-1) \text{ super-ratifies } b~ \vee$ 
        \State $(\exists b' \in \textit{blocklace}:\textit{height}(b') = d+w~ \wedge \textit{leader}(d+w) = b'.\textit{creator}~ \wedge b' \text{ ratifies } b $
        \State $\textit{blocklace\_prefix}(d+w) \text{ super-ratifies } b)$. 
         \EndProcedure
        
		
		\alglinenoPush{counter}
  \end{algorithmic}	
	\end{changemargin}
\end{algorithm}
\vspace{-2em}
\end{figure}


==> Code/tau.tex <==
\begin{figure}[t]
\begin{algorithm}[H] 
	\caption{\textbf{Mobile Consensus: Ordering of a Blocklace with $\boldsymbol{\tau}$} \\ pseudocode for miner $p$, including Algorithms \ref{alg:blocklace} 
	\& \ref{alg:MM}}
	\label{alg:tau}
	\small
	\begin{changemargin}{0cm}{-2cm}
	\begin{algorithmic}[1] 
	\alglinenoPop{counter} 

% 		\vspace{0.5em}
		\Statex \textbf{Local Variable:}
%         \StateX $\textit{slot} \gets 1$
		\StateX $\textit{outputBlocks} \gets \{\}$

% 		\vspace{0.5em}
		
		
	
		\label{alg:CMO:commitrule}
		
		 \Procedure{$\tau$}{$b_1$}: \label{alg:CMO:da}
		 	\If{$b_1 \in \textit{outputBlocks} \vee b_1 = \bot$}
		  \Return
		 \EndIf
		 \State  $b_2 \gets \textit{previous\_ratified\_block}(b_1)$
         \State  $\tau(b_2)$ \Comment{Recursive call to $\tau$}
		           
	  		  \State \textbf{output} $\textit{xsort}(b_1,[b_1] \setminus [b_2])$ \Comment{Output a new equivocation-free suffix} %\oded{Okazaki-fragment is not mentioned in the paper, only in a figure in the appendix. Can we remove it?}} 
	  		  \label{alg:CMO:Okazaki}
		      \State $\textit{outputBlocks} \gets \textit{outputBlocks} \cup \textit{xsort}(b_1,[b_1] \setminus [b_2])$
		  \EndProcedure
		 
        % \vspace{0.5em}
	    \Procedure{\textit{xsort}}{$b,B$}:  \Comment{Exclude equivocations and sort} 
	    \State \Return topological sort wrt $\succ$ of the set $\{b'\in B : \textit{approves}(b,b')\}$ 
	    \EndProcedure
	    
            % \vspace{0.5em}
		\Procedure{\textit{previous\_ratified\_block}}{$b_1$}: \label{alg:CMO:dr} \Comment{Fig. \ref{figure:approve-sr}.B}
              \State \Return $b \in [b_1]$ s.t. $b.\textit{payload}\ne \bot \wedge \textit{ratifies}(b_1,b) \wedge 
              (\exists b'\in [b_1] \wedge b'.\textit{payload}\ne \bot \wedge \textit{ratifies}(b_1,b') \implies  b'\not\succ b)$ 
        \EndProcedure 
	
        % \vspace{0.5em}
        % \Statex \textbf{procedure} 
        % is defined  Algorithm \ref{alg:protocols} 
	
        %\change{\State need to add a variant of this algorithm or two tau functions, one without a shared coin, and one with a shared coin for asynchrony.
		%The proofs for the blocklace-->blockchain need to accommodate the new tau function.}
	
	\alglinenoPush{counter}	
	\end{algorithmic}
	\end{changemargin}
\end{algorithm}
\vspace{-2em}

\end{figure}



==> multiagent.tex <==


\mypara{A Fault-Resilient Blocklace-Based Implementation}

A correct agent in the Flash payment system maintains a closed blocklace that only increases; initially has an initial block with input UTXOsan;  issues only balanced transactions; and does not equivocate.
An agent \emph{issues a block} by creating a block with its pending payments and pointers to the roots of it local blocklace, adding the block it to its blocklace and sending it to all agents except those known to be faulty. 

\udi{Not sure what to do about the following BPS.  It is a nice and simple formal specification.  But we need some definitions to be understood, and then the proof that the code implements it is informal.  So maybe leave it out/move to appendix?} \andy{I'd leave it out.}

\begin{definition}[BPS:  Blocklace Payment System]\label{definition:protocol-BPS}
The \temph{blocklace payment system} over $P$  is a distributed multiagent transition system $\textit{BPS}=(P,\textit{BX},T,\lambda)$ with transitions $T$  being all $p$-transitions $c\xrightarrow{}c'$, where $p \in P$, $c'_p= c_p \cup \{b\}$ and one of the following holds:
\begin{enumerate}[partopsep=0pt,topsep=0pt,parsep=0pt]
    \item \textbf{Pay}:   $b$ is $p$-block with a balanced transaction that has ratified inputs
    \item \textbf{Receive-$b$}: $b \in c_q\setminus c_p$ for some $q \in P$. 
\end{enumerate}
The liveness condition $\lambda$ partitions the $p$-transitions according to their labels.
\end{definition}

\begin{proposition}
The BPS transition system satisfies:
\begin{itemize}
    \item \textbf{Safety}:  No double-spending (how to formalize it here?)
    \item \textbf{Liveness}:  Every block known to a correct agent will be known to all
\end{itemize}
\end{proposition}
